On Quasi-Localized Dual Pairs in Reproducing Kernel Hilbert Spaces

In scattered data approximation, the span of a finite number of translates of a chosen radial basis function is used as approximation space and the basis of translates is used for representing the approximate. However, this natural choice is by no means mandatory and different choices, like, for example, the Lagrange basis, are possible and might offer additional features. In this article, we discuss different alternatives together with their canonical duals. We study a localized version of the Lagrange basis, localized orthogonal bases, such as the Newton basis, and multiresolution versions thereof, constructed by means of samplets. We argue that the choice of orthogonal bases is particularly useful as they lead to symmetric preconditioners. All bases under consideration are compared numerically to illustrate their feasibility for scattered data approximation. We provide benchmark experiments in two spatial dimensions and consider the reconstruction of an implicit surface as a relevant application from computer graphics.

==> Tables/Errors_d1_N1000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
        0.5    &        22      &  0.02265     &  0.0203001    &    9.57479 &  66.4317 \\
          1    &        43      & 0.04381      &  1.37238e-12  &    1.92816 &  4.18467 \\
        1.5    &        64      & 0.06472      &  1.14431e-12  &  0.778287  &  0.234652 \\
          2    &        85      & 0.085397     &  9.74486e-13  &  0.384037  &  0.0109767 \\
         2.5   &       105      & 0.105947     &  9.41793e-13  &  0.211419  &  0.000464597 \\
         3     &       125      & 0.125975     &  1.19655e-12  &  0.125941  &  1.63335e-05 \\
         3.5   &       145      & 0.145861     &  1.25826e-12  & 0.0788573  &  4.49522e-07 \\
         4     &       165      & 0.165922     &  1.42492e-12  & 0.0512793  &  3.10945e-08 \\
		}%		
\caption{Table of $ spec-err $ for $ N = 10^3$, $ \lambda = 10^{-6}$ in $ d = 1 $.}
\label{tab:d1_N1000}
\end{table}



==> Tables/Errors_d1_N10000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
        0.5    &     41         & 0.00411906   &  0.311517     & 24.8238    & 16.3645 \\
         1     &     81         & 0.00812562   & 0.000105903   & 67.9808    & 107.449 \\
        1.5    &    121         & 0.0121086    & 3.62613e-08   & 35.3296    & 165.587 \\
        2      &    160         & 0.0160886    & 1.08257e-11   & 15.6652    & 134.628 \\
        2.5    &    200         & 0.0200621    & 2.04376e-12   & 8.61949    & 77.8546 \\
        3      &    240         & 0.0240315    & 2.21311e-12   & 5.9116     & 32.7915 \\
        3.5    &    279         & 0.0279925    & 1.89138e-12   & 4.43183    & 6.6287  \\
        4      &    319         & 0.031939     & 2.01426e-12   & 3.42486    & 4.58391 \\
  		}%		
\caption{Table of $ spec-err $ for $ N = 10^4$, $ \lambda = 10^{-6}$ in $ d = 1 $.}
\label{tab:d1_N10000}
\end{table}

==> Tables/Errors_d1_N100000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
        0.5    &       63       & 0.000635789  &    222.483    &  331.361   &  348.825 \\
        1      &      126       & 0.0012616    &     52.483    & 154.311    & 170.359  \\
        1.5    &      188       & 0.00188611   &     13.1321   & 85.2405    &  106.852 \\
        2      &      251       & 0.00251101   &      3.29202  & 41.4785    & 70.5121  \\
        2.5    &      313       & 0.00313584   &     0.824962  & 8.36028    & 43.9572  \\
        3      &      376       & 0.00376024   &     0.206848  & 18.9483    & 21.6105  \\
  		}%		
\caption{Table of $ spec-err $ for $ N =10^5$, $ \lambda = 10^{-6}$ in $ d = 1 $.}
\label{tab:d1_N100000}
\end{table}

==> Tables/Errors_d2_N1000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
        0.5    &       17       & 0.017884     &     2.59537   &  3.02188      & 4.48555    \\
        1      &       64       & 0.06416      &    0.103989   &  0.0364512    & 0.162932  \\
        1.5    &      133       & 0.133476     &   0.0164087   &  0.00181752   & 0.00662425 \\
        2      &      218       & 0.218442     &  0.00360557   & 0.000403435   & 0.000359195 \\
        2.5    &      314       & 0.314844     &  0.00089673   & 0.000161731   & 4.0232e-05 \\
        3      &      418       & 0.418368     & 0.000239306   & 2.50578e-05   & 1.13117e-05\\
        % 3.5    &      523       & 0.523304     & 7.08501e-05   & 5.40728e-06   & 1.24218e-06\\
        % 4      &      625       & 0.62532      & 2.35292e-05   & 1.88325e-06    & 3.01652e-07\\ 
		}%		
\caption{Compression errors for $ N = 10^3$, $ \lambda = 10^{-6}$ in $ d = 2 $.}
\label{tab:d2_N1000}
\end{table}









==> Tables/Errors_d2_N10000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
          0.5  &         38     & 0.00388614   & 11.1651       &    2.68161 &     13.265 \\
            1  &        147     & 0.0147652    & 0.97808       &   0.259241 &    3.69366\\
          1.5  &        321     & 0.032132     & 0.277261      &  0.0194949 &   0.322787\\
            2  &        553     & 0.055357     & 0.101069      &   0.007955 &  0.0174833\\
          2.5  &        837     & 0.0837093    & 0.0423513     & 0.00346926 & 0.00415171\\
            3  &       1166     & 0.11663      & 0.0192898     & 0.00160194 & 0.00132455\\
%          3.5  &       1534     & 0.153457     & 0.00931418    & 0.000759778&0.000415133\\
%            4  &       1934     & 0.193469     & 0.00467335    & 0.000361902&0.000136823\\
		}%		
\caption{Compression errors for $ N = 10^4$, $ \lambda = 10^{-6}$ in $ d = 2 $.}
\label{tab:d2_N10000}
\end{table}

==> Tables/Errors_d2_N100000.tex <==
\begin{table}
\centering
	\pgfplotstabletypeset[
% 	font = \footnotesize,
		col sep=&, 
		row sep=\\,
		columns/kappa/.style={column name={ndof}, 1000 sep={\,}, fixed,column type = c},
  		columns/nFootprint/.style={column name={ndof}, fixed,},
    	columns/compression/.style={column name={ndof}, precision=5, fixed,column type = l},
		columns/nu05/.style={column name={$\nu=0.5$}, precision=3, zerofill,column type = l},
		columns/nu10/.style={column name={$\nu=1.0$}, precision=3, zerofill,column type = l},
		columns/nu15/.style={column name={$\nu=1.5$}, precision=3, zerofill,column type = l},
	%	every column/.style={column type=r},
		every head row/.style={
			output empty row,
            output empty row,
            output empty row,
            output empty row,
			before row={
				\toprule
				& \multicolumn{5}{c}{$ \operatorname{error} $}\\
				%
				\cmidrule(l){4-6}
				%
				\multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{$\kappa$} & \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{avg. $ \#X_j $} &
                \multicolumn{1}{@{}>{\columncolor{white}[0pt][\tabcolsep]}r}{comp. rate} &
                 $\nu=0.5$ & $\nu=1.0$ & $\nu=1.5$ \\
			},
			after row=\midrule
		},
		every last row/.style={after row=\bottomrule},
		every odd row/.style={before row={\rowcolor{gray!20}}},
		every first column/.style={column type/.add={@{}>{\columncolor{white}[0pt][\tabcolsep]}}{}},
		every last column/.style={column type/.add={>{\columncolor{white}[\tabcolsep][0pt]}}{@{}}},
		]{
		kappa  & nFootprint	 	&  compression & nu05          & nu10		& nu15 	  \\
      0.5      &     90         &  0.000906683 & 62.2871       &    266.423 &   448.263 \\
        1      &    354         & 0.00354691   &  6.03453      &    15.3282 &   21.1785 \\
      1.5      &    785         & 0.00785443   &  2.13354      &    0.57323 &   23.9281 \\
        2      &   1374         & 0.013747     &  0.960075     &  0.0877097 &   4.50762 \\
      2.5      &   2115         & 0.0211548    &  0.497623     &  0.0382435 &  0.527353 \\
        3      &   3000         & 0.0300006    &  0.281387     &  0.0207815 &   0.26966 \\
		}%		
\caption{Compression errors for $ N = 10^5$, $ \lambda = 10^{-6}$ in $ d = 2 $.}
\label{tab:d2_N100000}
\end{table}
